DIY e-HandPan: A new DIY Low-Cost Handpan Interface based on Arduino and ESP32 Microcontrollers

We present DIY e-HandPan, a new open-source, low-cost and customizable handpan audio and MIDI protocol interface designed for musical performance, education and research. The proposed hardware is built from inexpensive electronic components and recycled materials using widely available fabrication techniques, making it accessible to makers, educators and researchers. The instrument can be implemented on two distinct MicroController Unit (MCU): Arduino or ESP32. The microcontroller captures strike velocity to provide expressive musical performance comparable to that of an acoustic handpan. In addition to real-time audio and MIDI generation, DIY e-HandPan integrates a bi-color LED guidance system capable of displaying musical sequences from MIDI files, providing an effective learning aid for beginners and educational activities. The modular architecture allows users to easily customize the number of notes, hardware configuration and embedded software according to specific applications. We present the complete hardware design, firmware and assembly instructions and we discuss the design choices and limitations, to evaluate the system in representative educational and musical performance scenarios. All design files, source code and documentation are released under an open-source license to improve the reproducibility and encourage further developments by the open hardware community.

==> arduinofig2.tex <==
%\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[
    font=\sffamily,
    >=Latex,
    node distance=8mm and 13mm,

    block/.style={
        draw,
        rounded corners=2mm,
        align=center,
        minimum height=12mm,
        minimum width=32mm,
        inner sep=3mm,
        line width=0.8pt
    },

    smallblock/.style={
        draw,
        rounded corners=1.5mm,
        align=center,
        minimum height=9mm,
        minimum width=27mm,
        inner sep=2.5mm,
        line width=0.7pt
    },

    group/.style={
        draw,
        dashed,
        rounded corners=2mm,
        inner sep=4mm,
        line width=0.8pt
    },

    signal/.style={
        -{Latex[length=3mm]},
        line width=1.1pt
    },

    ledsignal/.style={
        -{Latex[length=3mm]},
        line width=1.1pt,
        dashed
    },

    bidirectional/.style={
        {Latex[length=3mm]}-{Latex[length=3mm]},
        line width=1.1pt
    },

    pad/.style={
        draw,
        ellipse,
        minimum width=8mm,
        minimum height=5mm,
        inner sep=0pt
    }
]

% ============================================================
% SALAD BOWL
% ============================================================

\node[
    draw,
    ellipse,
    minimum width=57mm,
    minimum height=38mm,
    line width=1pt,
    fill=gray!8
] (bowl) {};

\node[
    font=\bfseries,
    above=2mm of bowl
] {
    One salad bowl
};

\node[
    font=\small,
    below=1mm of bowl
] {
    6 or 8 notes
};

% Playing surfaces
\foreach \angle in {0,45,...,315}{
    \node[pad]
        at ($(bowl.center)+(\angle:18mm)$) {};
}

\node[
    smallblock,
    below=11mm of bowl,
    minimum width=45mm
] (notehardware) {
    \textbf{Per-note hardware}\\
    One piezoelectric sensor\\
    One red/green bi-color LED
};

% ============================================================
% UPPER PATH: PIEZO ACQUISITION
% Bowl -> conditioning -> connection 1 -> Arduino
% ============================================================

\node[
    smallblock,
    right=18mm of bowl,
    yshift=13mm,
    minimum width=38mm
] (conditioning) {
    \textbf{Signal conditioning}\\
    One circuit per piezo\\
    See dedicated schematic
};

\node[
    smallblock,
    right=17mm of conditioning,
    minimum width=39mm
] (connectionPiezo) {
    \textbf{Optional connection 1}\\
    DB25 or RJ45 cables\\
    Piezo signal path
};

% Bowl -> conditioning
\draw[signal]
    ($(bowl.east)+(0,9mm)$)
    --
    node[
        above,
        font=\small,
        align=center
    ] {
        raw piezo\\
        signals
    }
    (conditioning.west);

% Conditioning -> optional connection 1
\draw[signal]
    (conditioning.east)
    --
    node[
        above,
        font=\small,
        align=center
    ] {
        conditioned\\
        outputs
    }
    (connectionPiezo.west);

% ============================================================
% LOWER PATH: LED CONTROL
% Arduino -> connection 2 -> resistors -> bowl
% ============================================================

\node[
    smallblock,
    right=18mm of bowl,
    yshift=-14mm,
    minimum width=38mm
] (resistors) {
    \textbf{LED protection}\\
    100~$\Omega$ series resistor\\
    on each control line
};

\node[
    smallblock,
    right=17mm of resistors,
    minimum width=39mm
] (connectionLED) {
    \textbf{Optional connection 2}\\
    DB25 or RJ45 cables\\
    LED control path
};

% Optional connection 2 -> resistors
\draw[ledsignal]
    (connectionLED.west)
    --
    node[
        below,
        font=\small,
        align=center
    ] {
        LED control\\
        lines
    }
    (resistors.east);

% Resistors -> bowl
\draw[ledsignal]
    (resistors.west)
    --
    node[
        below,
        font=\small,
        align=center
    ] {
        protected LED\\
        inputs
    }
    ($(bowl.east)+(0,-9mm)$);

% ============================================================
% GROUPS
% ============================================================

\node[
    group,
    fit=(conditioning)(connectionPiezo),
    label={[font=\bfseries]above:Piezo acquisition path}
] (piezoGroup) {};

\node[
    group,
    fit=(resistors)(connectionLED),
    label={[font=\bfseries]below:LED control path}
] (ledGroup) {};

% ============================================================
% ARDUINO
% ============================================================

\node[
    block,
    right=23mm of connectionPiezo,
    yshift=-3mm,
    minimum width=50mm,
    minimum height=69mm,
    align=left
] (arduino) {
    \textbf{\large Arduino Uno / Mega}\\[2mm]
    $\bullet$ Direct analog acquisition\\
    $\bullet$ Impact detection\\
    $\bullet$ Velocity estimation\\
    $\bullet$ MIDI Note On/Off generation\\
    $\bullet$ Incoming MIDI decoding\\
    $\bullet$ Bi-color LED control\\
    $\bullet$ MocoLUFA USB-MIDI interface
};

% Connection 1 -> Arduino
\draw[signal]
    (connectionPiezo.east)
    --
    node[
        above,
        font=\small,
        align=center
    ] {
        conditioned analog\\
        signals
    }
    (arduino.west |- connectionPiezo.east);

% Arduino -> connection 2
\draw[ledsignal]
    (arduino.west |- connectionLED.east)
    --
    node[
        below,
        font=\small,
        align=center
    ] {
        LED control\\
        outputs
    }
    (connectionLED.east);

% ============================================================
% ANALOG INPUT NOTE
% ============================================================

\node[
    draw,
    rounded corners,
    align=left,
    font=\footnotesize,
    above=8mm of arduino,
    minimum width=51mm
] (analogNote) {
    \textbf{Direct sensor acquisition}\\
    Arduino Uno: 6 or 8 notes, one bowl\\
    Arduino Mega: 14 notes, two bowls\\
    No analog multiplexer is required
};

\draw[
    dashed,
    -{Latex[length=2.5mm]}
]
    (analogNote.south)
    --
    (arduino.north);

% ============================================================
% COMPUTER / MIDI HOST
% ============================================================

\node[
    block,
    right=23mm of arduino,
    minimum width=52mm,
    minimum height=69mm,
    align=left
] (computer) {
    \textbf{\large Computer / MIDI host}\\[2mm]
    $\bullet$ Software sound expander\\
    $\bullet$ Handpan sound library\\
    $\bullet$ Educational MIDI player\\
    $\bullet$ MIDI file loading\\
    $\bullet$ Tempo and loop control\\
    $\bullet$ Left/right-hand information
};

\draw[bidirectional]
    (arduino.east)
    --
    node[
        above,
        align=center,
        font=\small
    ] {
        USB-MIDI\\
        MocoLUFA
    }
    (computer.west);

% ============================================================
% AUDIO OUTPUT
% ============================================================

\node[
    smallblock,
    right=17mm of computer,
    yshift=15mm,
    minimum width=36mm
] (audio) {
    \textbf{Audio output}\\
    Computer sound card\\
    headphones or speaker
};

\draw[signal]
    (computer.east |- audio.west)
    --
    node[
        above,
        font=\small
    ] {
        audio
    }
    (audio.west);

% ============================================================
% EDUCATIONAL MIDI FILE
% ============================================================

\node[
    smallblock,
    right=17mm of computer,
    yshift=-20mm,
    minimum width=38mm
] (midifile) {
    \textbf{Educational MIDI file}\\
    Notes and timing\\
    Left/right-hand information
};

% MIDI file -> computer
\draw[signal]
    (midifile.west)
    --
    node[
        below,
        font=\small
    ] {
        MIDI sequence
    }
    (computer.east |- midifile.west);

% ============================================================
% FIRMWARE TASKS
% ============================================================

\node[
    draw,
    rounded corners,
    align=center,
    font=\footnotesize,
    below=14mm of arduino,
    minimum width=58mm
] (firmwareFlow) {
    \textbf{Simultaneous firmware tasks}\\[1mm]
    Piezo impacts $\rightarrow$ velocity-sensitive MIDI messages\\
    Incoming MIDI messages $\rightarrow$ LED guidance
};

\draw[
    dashed,
    -{Latex[length=2.5mm]}
]
    (arduino.south)
    --
    (firmwareFlow.north);

% ============================================================
% LEGEND
% ============================================================

\node[
    draw,
    rounded corners,
    align=left,
    font=\footnotesize,
    below=20mm of notehardware,
    anchor=north west,
    minimum width=74mm
] (legend) {
    \textbf{Functional signal flows}\\[1mm]
    Piezo: bowl $\rightarrow$ conditioning $\rightarrow$
    connection 1 $\rightarrow$ Arduino\\
    LED: Arduino $\rightarrow$ connection 2 $\rightarrow$
    100~$\Omega$ resistors $\rightarrow$ bowl\\
    MIDI: Arduino $\leftrightarrow$ computer
};

\end{tikzpicture}%
%}

==> esp32fig.tex <==
\!\!\!\resizebox{1.05\textwidth}{!}{%
\begin{tikzpicture}[
    font=\sffamily,
    >=Latex,
    node distance=8mm and 12mm,
    block/.style={
        draw,
        rounded corners=2mm,
        align=center,
        minimum height=12mm,
        minimum width=30mm,
        inner sep=3mm,
        line width=0.8pt
    },
    smallblock/.style={
        draw,
        rounded corners=1.5mm,
        align=center,
        minimum height=9mm,
        minimum width=25mm,
        inner sep=2mm,
        line width=0.7pt
    },
    group/.style={
        draw,
        dashed,
        rounded corners=2mm,
        inner sep=4mm,
        line width=0.8pt
    },
    signal/.style={
        -{Latex[length=3mm]},
        line width=1.1pt
    },
    bidirectional/.style={
        {Latex[length=3mm]}-{Latex[length=3mm]},
        line width=1.1pt
    },
    pad/.style={
        draw,
        ellipse,
        minimum width=8mm,
        minimum height=5mm,
        inner sep=0pt
    }
]

% ============================================================
% HANDPAN
% ============================================================

\node[
    draw,
    ellipse,
    minimum width=55mm,
    minimum height=37mm,
    line width=1pt,
    fill=gray!8
] (handpan) {};

\node[font=\bfseries, above=2mm of handpan]
    {DIY eHandPan};

\node[font=\small, below=1mm of handpan]
    {14 playing surfaces};

% Central pad
\node[pad, minimum width=11mm, minimum height=7mm]
    at (handpan.center) {};

% Outer pads
\foreach \angle in {0,45,...,315}{
    \node[pad]
        at ($(handpan.center)+(\angle:18mm)$) {};
}

% Inner pads
\foreach \angle in {22.5,82.5,...,322.5}{
    \node[pad, minimum width=7mm, minimum height=4mm]
        at ($(handpan.center)+(\angle:11mm)$) {};
}

% Piezo and LED labels
\node[
    smallblock,
    below=11mm of handpan,
    minimum width=42mm
] (sensors) {
    \textbf{Per-note hardware}\\
    14 piezoelectric sensors\\
    14 red/green bi-color LEDs
};

\draw[signal]
    (handpan.south) -- (sensors.north);

% ============================================================
% DB25 CONNECTION
% ============================================================

\node[
    block,
    right=17mm of handpan,
    minimum width=23mm,
    minimum height=34mm
] (db25) {
    \textbf{DB25}\\[0.5mm]
    Piezo signals\\
    LED lines\\
    Power and ground
};

\draw[bidirectional]
    (handpan.east) --
    node[above, align=center, font=\small]
    {DB25 cable}
    (db25.west);

% ============================================================
% INTERFACE BOARD
% ============================================================

\node[
    smallblock,
    right=18mm of db25,
    yshift=11mm
] (mux) {
    \textbf{CD4067}\\
    16-channel\\
    analog MUX
};

\node[
    smallblock,
    right=18mm of db25,
    yshift=-12mm
] (shift) {
    \textbf{74HC595}\\
    cascaded\\
    shift registers
};

\node[
    group,
    fit=(mux)(shift),
    label={[font=\bfseries]above:Interface board}
] (interface) {};

\draw[signal]
    (db25.east |- mux.west) --
    node[above, font=\small]
    {piezo signals}
    (mux.west);

\draw[signal]
    (shift.west) --
    node[below, font=\small]
    {LED signals}
    (db25.east |- shift.west);

% ============================================================
% ESP32
% ============================================================

\node[
    block,
    right=25mm of interface,
    minimum width=48mm,
    minimum height=62mm,
    align=left
] (esp32) {
    \textbf{\large ESP32-S3-N16R8}\\[2mm]
    $\bullet$ Impact detection\\
    $\bullet$ Velocity estimation\\
    $\bullet$ Audio sample playback\\
    $\bullet$ MIDI file processing\\
    $\bullet$ LED learning sequences\\
    $\bullet$ Embedded HTTP server\\
    $\bullet$ Wi-Fi access point
};

\draw[signal]
    (mux.east) --
    node[above, font=\small, align=center]
    {Multiplexed\\analog input}
    (esp32.west |- mux.east);

\draw[signal]
    (esp32.west |- shift.east) --
    node[below, font=\small, align=center]
    {Serial LED\\control}
    (shift.east);

% ADC note
\node[
    draw,
    rounded corners,
    align=left,
    font=\footnotesize,
    above=8mm of esp32,
    minimum width=50mm
] (adcnote) {
    \textbf{Analog-input constraint}\\
    18 ADC-capable inputs available on the platform\\
    10 pins reserved or unavailable in this design\\
    $\Rightarrow$ analog multiplexing used for 14 notes
};

\draw[
    dashed,
    -{Latex[length=2.5mm]}
] (adcnote.south) -- (esp32.north);

% ============================================================
% MEMORY
% ============================================================

\node[
    smallblock,
    below=11mm of esp32,
    minimum width=47mm
] (memory) {
    \textbf{Flash memory / PSRAM}\\
    WAV handpan samples\\
    MIDI files, firmware and settings
};

\draw[bidirectional]
    (esp32.south) --
    node[right, font=\small]
    {data}
    (memory.north);

% ============================================================
% AUDIO OUTPUT
% ============================================================

\node[
    smallblock,
    right=20mm of esp32,
    yshift=13mm
] (dac) {
    \textbf{UDA1334A DAC}\\
    I$^2$S digital-to-analog\\
    conversion
};

\node[
    smallblock,
    right=14mm of dac,
    minimum width=31mm
] (audio) {
    \textbf{Audio output}\\
    3.5-mm jack\\
    headphones / speaker
};

\draw[signal]
    (esp32.east |- dac.west) --
    node[above, font=\small]
    {I$^2$S}
    (dac.west);

\draw[signal]
    (dac.east) --
    node[above, font=\small]
    {analog audio}
    (audio.west);

% ============================================================
% WEB INTERFACE
% ============================================================

\node[
    smallblock,
    right=20mm of esp32,
    yshift=-26mm,
    minimum width=47mm
] (web) {
    \textbf{User Web interface}\\
    Smartphone, tablet or computer\\[1mm]
    MIDI file upload\\
    Tempo and loop configuration\\
    Learning-mode selection\\
    Instrument configuration
};

\draw[
    bidirectional,
    dashed
]
    (esp32.east |- web.west) --
    node[above, font=\small, align=center]
    {Wi-Fi / HTTP}
    (web.west);

% ============================================================
% FUNCTIONAL FLOW LABELS
% ============================================================

\node[
    align=center,
    font=\footnotesize,
    below=5mm of interface
] {
    The MUX acquires the piezo signals;\\
    the shift registers independently drive the LEDs.
};

\node[
    align=center,
    font=\footnotesize,
    below=6mm of audio
] {
    Pre-recorded handpan samples\\
    are played after impact detection.
};

% ============================================================
% LEGEND
% ============================================================

\node[
    draw,
    rounded corners,
    align=left,
    font=\footnotesize,
    below=19mm of sensors,
    anchor=north west,
    minimum width=66mm
] (legend) {
    \textbf{Signal-flow legend}\\[1mm]
    $\longrightarrow$ Piezoelectric sensor data\\
    $\longleftarrow$ LED control data\\
    $\longleftrightarrow$ Bidirectional communication
};

\end{tikzpicture}%
}


==> figs/arduinofig.tex <==
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[
    font=\sffamily,
    >=Latex,
    node distance=8mm and 13mm,
    block/.style={
        draw,
        rounded corners=2mm,
        align=center,
        minimum height=12mm,
        minimum width=32mm,
        inner sep=3mm,
        line width=0.8pt
    },
    smallblock/.style={
        draw,
        rounded corners=1.5mm,
        align=center,
        minimum height=9mm,
        minimum width=27mm,
        inner sep=2.5mm,
        line width=0.7pt
    },
    group/.style={
        draw,
        dashed,
        rounded corners=2mm,
        inner sep=4mm,
        line width=0.8pt
    },
    signal/.style={
        -{Latex[length=3mm]},
        line width=1.1pt
    },
    bidirectional/.style={
        {Latex[length=3mm]}-{Latex[length=3mm]},
        line width=1.1pt
    },
    pad/.style={
        draw,
        ellipse,
        minimum width=8mm,
        minimum height=5mm,
        inner sep=0pt
    }
]

% ============================================================
% EHANDPAN
% ============================================================

\node[
    draw,
    ellipse,
    minimum width=57mm,
    minimum height=38mm,
    line width=1pt,
    fill=gray!8
] (handpan) {};

\node[font=\bfseries, above=2mm of handpan]
    {DIY eHandPan};

\node[font=\small, below=1mm of handpan]
    {6-, 8-, or 14-note configuration};

% Central playing surface
\node[
    pad,
    minimum width=11mm,
    minimum height=7mm
] at (handpan.center) {};

% Playing surfaces
\foreach \angle in {0,45,...,315}{
    \node[pad]
        at ($(handpan.center)+(\angle:18mm)$) {};
}

\foreach \angle in {22.5,82.5,...,322.5}{
    \node[
        pad,
        minimum width=7mm,
        minimum height=4mm
    ] at ($(handpan.center)+(\angle:11mm)$) {};
}

\node[
    smallblock,
    below=11mm of handpan,
    minimum width=45mm
] (notehardware) {
    \textbf{Per-note hardware}\\
    Piezoelectric sensor\\
    Red/green bi-color LED
};

\draw[signal]
    (handpan.south) -- (notehardware.north);

% ============================================================
% TWO RJ45 CONNECTIONS
% ============================================================

\node[
    block,
    right=18mm of handpan,
    yshift=10mm,
    minimum width=28mm
] (rj45a) {
    \textbf{RJ45 cable 1}\\
    Bowl A\\
    up to 8 piezos\\
    common ground
};

\node[
    block,
    right=18mm of handpan,
    yshift=-17mm,
    minimum width=28mm
] (rj45b) {
    \textbf{RJ45 cable 2}\\
    Bowl B\\
    up to 6 piezos\\
    common ground
};

\draw[bidirectional]
    ($(handpan.east)+(0,6mm)$) --
    node[above, font=\small]
    {sensor and LED wiring}
    (rj45a.west);

\draw[bidirectional]
    ($(handpan.east)+(0,-7mm)$) --
    (rj45b.west);

% ============================================================
% SIGNAL CONDITIONING
% ============================================================

\node[
    smallblock,
    right=17mm of rj45a,
    minimum width=37mm
] (conditioningA) {
    \textbf{Signal conditioning}\\
    Protection circuit\\
    or $R_1$ in parallel
};

\node[
    smallblock,
    right=17mm of rj45b,
    minimum width=37mm
] (conditioningB) {
    \textbf{Signal conditioning}\\
    Protection circuit\\
    or $R_1$ in parallel
};

\draw[signal]
    (rj45a.east) -- (conditioningA.west);

\draw[signal]
    (rj45b.east) -- (conditioningB.west);

\node[
    group,
    fit=(conditioningA)(conditioningB),
    label={[font=\bfseries]above:Piezoelectric input stage}
] (conditioninggroup) {};

% ============================================================
% ARDUINO
% ============================================================

\node[
    block,
    right=22mm of conditioninggroup,
    minimum width=48mm,
    minimum height=68mm,
    align=left
] (arduino) {
    \textbf{\large Arduino Uno / Mega}\\[2mm]
    $\bullet$ Direct analog acquisition\\
    $\bullet$ Impact detection\\
    $\bullet$ Velocity estimation\\
    $\bullet$ MIDI Note On/Off generation\\
    $\bullet$ Incoming MIDI decoding\\
    $\bullet$ Bi-color LED control\\
    $\bullet$ MocoLUFA USB-MIDI interface
};

\draw[signal]
    (conditioningA.east) --
    node[above, font=\small]
    {analog inputs}
    (arduino.west |- conditioningA.east);

\draw[signal]
    (conditioningB.east) --
    node[below, font=\small]
    {analog inputs}
    (arduino.west |- conditioningB.east);

% Analog input note
\node[
    draw,
    rounded corners,
    align=left,
    font=\footnotesize,
    above=8mm of arduino,
    minimum width=51mm
] (analogNote) {
    \textbf{Direct sensor acquisition}\\
    Arduino Uno: up to 8 analog inputs\\
    Arduino Mega: up to 14 sensors used here\\
    No analog multiplexer is required
};

\draw[
    dashed,
    -{Latex[length=2.5mm]}
]
    (analogNote.south) -- (arduino.north);

% ============================================================
% LED RETURN PATH
% ============================================================

\draw[signal]
    ($(arduino.west)+(0,-20mm)$)
    -- ++(-8mm,0)
    |- 
    node[pos=0.72, below, font=\small]
    {LED control lines}
    (rj45b.east);

% ============================================================
% COMPUTER / MIDI HOST
% ============================================================

\node[
    block,
    right=23mm of arduino,
    minimum width=52mm,
    minimum height=69mm,
    align=left
] (computer) {
    \textbf{\large Computer / MIDI host}\\[2mm]
    $\bullet$ Software sound expander\\
    $\bullet$ Handpan sound library\\
    $\bullet$ MIDI file player\\
    $\bullet$ Tempo and song selection\\
    $\bullet$ Educational score playback
};

\draw[bidirectional]
    (arduino.east) --
    node[
        above,
        align=center,
        font=\small
    ]
    {USB-MIDI\\MocoLUFA}
    (computer.west);

% ============================================================
% AUDIO OUTPUT
% ============================================================

\node[
    smallblock,
    right=17mm of computer,
    yshift=15mm,
    minimum width=36mm
] (audio) {
    \textbf{Audio output}\\
    Computer sound card\\
    headphones / speaker
};

\draw[signal]
    (computer.east |- audio.west) --
    node[above, font=\small]
    {audio}
    (audio.west);

% ============================================================
% MIDI LEARNING FLOW
% ============================================================

\node[
    smallblock,
    right=17mm of computer,
    yshift=-20mm,
    minimum width=38mm
] (midifile) {
    \textbf{Educational MIDI file}\\
    Notes and timing\\
    Left/right-hand information
};

\draw[signal]
    (midifile.west) --
    node[below, font=\small]
    {MIDI sequence}
    (computer.east |- midifile.west);

% ============================================================
% FLOW LABELS
% ============================================================

\node[
    draw,
    rounded corners,
    align=center,
    font=\footnotesize,
    below=13mm of arduino,
    minimum width=55mm
] (firmwareflow) {
    \textbf{Simultaneous firmware tasks}\\[1mm]
    Sensors $\rightarrow$ velocity-aware MIDI messages\\
    Incoming MIDI messages $\rightarrow$ LED guidance
};

\draw[
    dashed,
    -{Latex[length=2.5mm]}
]
    (arduino.south) -- (firmwareflow.north);

% ============================================================
% LEGEND
% ============================================================

\node[
    draw,
    rounded corners,
    align=left,
    font=\footnotesize,
    below=20mm of notehardware,
    anchor=north west,
    minimum width=69mm
] (legend) {
    \textbf{Functional signal flows}\\[1mm]
    Piezo strike $\rightarrow$ analog signal $\rightarrow$ MIDI event\\
    MIDI player $\rightarrow$ Arduino $\rightarrow$ illuminated LED\\
    MIDI event $\rightarrow$ software expander $\rightarrow$ audio
};

\end{tikzpicture}%
}


